The Variational Quantum Eigensolver: a review of methods and best practices

The variational quantum eigensolver (or VQE) uses the variational principle to compute the ground state energy of a Hamiltonian, a problem that is central to quantum chemistry and condensed matter physics. Conventional computing methods are constrained in their accuracy due to the computational limits. The VQE may be used to model complex wavefunctions in polynomial time, making it one of the most promising near-term applications for quantum computing. Finding a path to navigate the relevant literature has rapidly become an overwhelming task, with many methods promising to improve different parts of the algorithm. Despite strong theoretical underpinnings suggesting excellent scaling of individual VQE components, studies have pointed out that their various pre-factors could be too large to reach a quantum computing advantage over conventional methods. This review aims to provide an overview of the progress that has been made on the different parts of the algorithm. All the different components of the algorithm are reviewed in detail including representation of Hamiltonians and wavefunctions on a quantum computer, the optimization process, the post-processing mitigation of errors, and best practices are suggested. We identify four main areas of future research:(1) optimal measurement schemes for reduction of circuit repetitions; (2) large scale parallelization across many quantum computers;(3) ways to overcome the potential appearance of vanishing gradients in the optimization process, and how the number of iterations required for the optimization scales with system size; (4) the extent to which VQE suffers for quantum noise, and whether this noise can be mitigated. The answers to these open research questions will determine the routes for the VQE to achieve quantum advantage as the quantum computing hardware scales up and as the noise levels are reduced.

==> 10_List_of_symbols.tex <==
% Note:
% At the moment 
% command format: 
% 1. \nomenclature[grouping-prefix]{symbol}{description}
% The grouping-prefix helps to sort the symbols: Symbols will be sorted by <prefox><symbol>. 

% defines the title of the list of symbols:
\renewcommand{\nomname}{List of Symbols}
% a short introduction to this section:
\renewcommand{\nompreamble}{Here lists several symbols that are used in this paper.}

% Grouping convention (Juat a first try, haven't figure out the best way to do it yet:
% c: small symbols
% g: Matrix and operators
% l: complex expressions.

\nomenclature[g]{$\hat{H}$}{Hamiltonian of the quantum mechanical system.}
\nomenclature[g]{$\hat{P_a}$}{Any Pauli operator or tensor of Pauli operators (Pauli string)}
\nomenclature[c]{$n$}{Number of basis functions used for in the Hamiltonian. It can also refer to, the number of fermionic modes, or the number of site on a lattice}
\nomenclature[c]{$m$}{The number of electrons in the system of interest}
\nomenclature[c]{$N$}{Refers to the number of qubits used to model the wavefunction of the system of interest}
\nomenclature[c]{$\epsilon$}{A given level of precision, i.e. the maximum error in estimation. A variant of this symbol, $\varepsilon$, is used to represent the level of noise in the quantum computer.}
\nomenclature[l]{$\mathcal{O}(f(n))$}{Order of function $f(n)$.}
\nomenclature[g]{$\unit$}{The identity matrix of an appropriate dimension.}
\nomenclature[g]{$I$}{The $2$ by $2$ identity matrix.}
\nomenclature[g]{$X/Y/Z$}{The three $2$ by $2$ Pauli $X$, Pauli-$Y$ and Pauli-$Z$ matrices.}
\nomenclature[g]{$\mathcal{P}$}{The number of Pauli strings in a Hamiltonian.}
\nomenclature[g]{$\hat{P}$}{Any Pauli string.}
\nomenclature[l]{$\phi_i(.)$, $\ket{\phi_i}$}{A spin-orbital function}
\nomenclature[l]{$\psi(.)$, $\ket{\psi}$}{An electronic wavefunction}

\printnomenclature

